Hamiltonian Cycle Parameterized by Treedepth in Single Exponential Time and Polynomial Space

For many algorithmic problems on graphs of treewidth $t$, a standard dynamic programming approach gives an algorithm with time and space complexity $2^{\mathcal{O}(t)}\cdot n^{\mathcal{O}(1)}$. It turns out that when one considers the more restrictive parameter treedepth, it is often the case that a variation of this technique can be used to reduce the space complexity to polynomial, while retaining time complexity of the form $2^{\mathcal{O}(d)}\cdot n^{\mathcal{O}(1)}$, where $d$ is the treedepth. This transfer of methodology is, however, far from automatic. For instance, for problems with connectivity constraints, standard dynamic programming techniques give algorithms with time and space complexity $2^{\mathcal{O}(t\log t)}\cdot n^{\mathcal{O}(1)}$ on graphs of treewidth $t$, but it is not clear how to convert them into time-efficient polynomial space algorithms for graphs of low treedepth. Cygan et al. (FOCS'11) introduced the Cut&Count technique and showed that a certain class of problems with connectivity constraints can be solved in time and space complexity $2^{\mathcal{O}(t)}\cdot n^{\mathcal{O}(1)}$. Recently, Hegerfeld and Kratsch (STACS'20) showed that, for some of those problems, the Cut&Count technique can be also applied in the setting of treedepth, and it gives algorithms with running time $2^{\mathcal{O}(d)}\cdot n^{\mathcal{O}(1)}$ and polynomial space usage. However, a number of important problems eluded such a treatment, with the most prominent examples being Hamiltonian Cycle and Longest Path. In this paper we clarify the situation by showing that Hamiltonian Cycle, Hamiltonian Path, Long Cycle, Long Path, and Min Cycle Cover all admit $5^d\cdot n^{\mathcal{O}(1)}$-time and polynomial space algorithms on graphs of treedepth $d$. The algorithms are randomized Monte Carlo with only false negatives.

==> Makefile <==
SOURCES := $(shell find $(SOURCEDIR) -name '*.tex')

all: main.pdf

main.pdf: $(SOURCES) main.bbl 
	pdflatex main.tex
	pdflatex main.tex

main.aux: $(SOURCES)
	pdflatex main.tex

main.bbl: bib.bib main.aux
	bibtex main

clean:
	rm -f img/*.log img/*.aux img/*.pdf
	rm -f *~ *.log *.out *.aux *.blg *.bbl *.gz

distclean: clean
	rm -f main.pdf

tar: clean
	bash -c "cd ..; tar -czf ${BASE}.tar.gz ${BASE}/*; mv ${BASE}.tar.gz ${BASE}"

spell:
	@for i in `find . -name "*.tex"` ; do \
		echo "------------ $$i --------------" ; \
		aspell list --lang=en --mode=tex --dont-tex-check-comments --personal=./blue-slownik.txt < $$i | sort | uniq ; \
done

diff:
	mkdir /tmp/cut-and-count-diff/
	python2 ~/latex-flatten.py main.tex /tmp/cut-and-count-diff/test.tex
	python2 ~/latex-flatten.py /tmp/cut-and-count-diff/test.tex /tmp/cut-and-count-diff/test2.tex
	python2 ~/latex-flatten.py /tmp/cut-and-count-diff/test2.tex /tmp/cut-and-count-diff/d2.tex
	git checkout $(branch-id)
	python2 ~/latex-flatten.py main.tex /tmp/cut-and-count-diff/test.tex
	python2 ~/latex-flatten.py /tmp/cut-and-count-diff/test.tex /tmp/cut-and-count-diff/test2.tex
	python2 ~/latex-flatten.py /tmp/cut-and-count-diff/test2.tex /tmp/cut-and-count-diff/d1.tex
	latexdiff /tmp/cut-and-count-diff/d1.tex /tmp/cut-and-count-diff/d2.tex > /tmp/cut-and-count-diff/diff.tex
	pdflatex /tmp/cut-and-count-diff/diff.tex
	git checkout master


==> chapters/cut-and-count.tex <==
\section{Cut\&Count}

\karol{This section presents a short introduction to Cut\&Count. I am not sure
where should it be}


In this section, we will briefly overview the Cut\&Count technique. Imagine you
have a connectivity problem, with the set of solutions $\mathcal{S} \subseteq
2^U$. Your goal is to decide if $\mathcal{S}$ is empty or not. In our
applications, set $U$ is just a set of edges.

Conceptually, Cut\&Count technique consists of two steps:

\begin{itemize}

    \item \textbf{Cut part}: Relax the problem by considering the set
        $\mathcal{R} \supseteq \mathcal{S}$ of many, possibly disconnected
        candidate solutions. Furthermore, we would like to choose choose
        candidate set to preserve the parity of $|\mathcal{S}$. We achieve it by
        considering set $\mathcal{C}$ of pairs $(X,C)$, where $X \in
        \mathcal{R}$ and $C$ is a consistent cut of $X$.

    \item \textbf{Count part}: Compute $|\mathcal{C}|$ modulo 2. We hope that
        this step should be simple to compute, since we significantly relaxed
        our candidate set. Moreover, disconnected solutions in
        $\mathcal{R}\setminus \mathcal{C}$ should cancel-out modulo 2, since
        they are consistent with an even number of cuts. For example cycle cover
        of exactly $k$ disconnected cycles is consistent with exactly $2^k$
        cuts.
\end{itemize}

Note, that we need $|\mathcal{S}|$ to be odd in the first place, for the
procedure to work. We can guarantee this with Isolation Lemma. It comes at a
cost of counting \emph{weighted} solutions modulo 2. This step, as it often
turns out is not that computationally expensive.

For every element $v \in U$ we choose uniformly at random weight $\omega(v)$.
Then, for every $w \in \{1, \ldots, 2|U|^2\}$ we compute $|\mathcal{C}_w|$
modulo 2, where $\mathcal{C}_w = \{(X,C) \in \mathcal{C} \; | \; \omega(X) =
w\}$. We return \textbf{yes} iff for some $w$ we have that $|\mathcal{C}_w|
\equiv_2 1$. The general schema of Cut\&Count is presented below.

\begin{algorithm}
\SetAlgoLined
\ForEach{$e \in E(G)$}{
    Select $\omega(e)$ uniformly at random from $\{1,\ldots,2|E(G)|\}$
}
\ForEach{$w \in \{1,\ldots,2|E(G)|^2\}$}{
    Count $|\mathcal{C}_w|$ modulo $2^c$.\\
    \If{ $|\mathcal{C}_w| \not\equiv 0 \Mod{2^c}$ }{
        Return \textbf{Yes}
    }
}
Return \textbf{No}
\caption{General approach to Cut \& Count}
\label{CutAndCount}
\end{algorithm}

The correctness of Algorithm~\ref{CutAndCount} is summarized by the following
Corollary from Isolation Lemma.

\begin{corollary}[\cite{focs2011}]
    Let $\mathcal{S} \subseteq 2^E$ and $\mathcal{C} \subseteq 2^U \times (2^V
    \times 2^V)$ and $c \in \nat$. Suppose that for every $w \in \nat$

    \begin{displaymath}
        |\{ (X,C) \in \mathcal{C} \; | \; \omega(X) = w \}| \equiv | \{ X \in \mathcal{S} \; | \; \omega(X) = w\} | \Mod{2^c}.
    \end{displaymath}

    Then Algorithm~\ref{CutAndCount} returns \textbf{No} if $\mathcal{S}$ is
    empty and otherwise returns \textbf{Yes} with probability at least
    $\frac{1}{2}$.
\end{corollary}

In our approach we will need $c$ to be at least $n+k+1$. We can allow this
because arithmetic operations modulo $2^{\Oh(n)}$ incur only polynomial
overhead.

